Parameterized Complexity of Minimum Membership Dominating Set

Given a graph $G=(V,E)$ and an integer $k$, the Minimum Membership Dominating Set (MMDS) problem seeks to find a dominating set $S \subseteq V$ of $G$ such that for each $v \in V$, $|N[v] \cap S|$ is at most $k$. We investigate the parameterized complexity of the problem and obtain the following results about MMDS: W[1]-hardness of the problem parameterized by the pathwidth (and thus, treewidth) of the input graph. W[1]-hardness parameterized by $k$ on split graphs. An algorithm running in time $2^{\mathcal{O}(\textbf{vc})} |V|^{\mathcal{O}(1)}$, where $\textbf{vc}$ is the size of a minimum-sized vertex cover of the input graph. An ETH-based lower bound showing that the algorithm mentioned in the previous item is optimal.

==> commands.tex <==
\newcommand{\zigzag}{zigzag}

\newcommand{\bli}{\textbf{i}}
\newcommand{\blj}{\textbf{j}}
\newcommand{\blh}{\textbf{h}}
\newcommand{\blr}{\textbf{r}}
\newcommand{\ca}{\alpha}
\newcommand{\cb}{\beta}
\newcommand{\cd}{\lambda}
\newcommand{\cons}{\textsc{Cons}}
\newcommand{\inv}{^{-1}}
\newcommand{\sol}{\texttt{Sol}}
\newcommand{\soli}{\texttt{Sol}_\bli}
\newcommand{\solj}{\texttt{Sol}_\blj}
\newcommand{\solh}{\texttt{Sol}_\blh}
%\newcommand{\tw}{w}
\newcommand{\val}{\texttt{Val}}
\newcommand{\vali}{\texttt{Val}_\bli}
\newcommand{\valj}{\texttt{Val}_\blj}
\newcommand{\valh}{\texttt{Val}_\blh}

\newcommand{\Gi}{\G[\Xi^+]}
\newcommand{\Ci}{\C_{\Gi}}
\newcommand{\Gj}{\G[\Xj^+]}
\newcommand{\Cj}{\C_{\Gj}}
\newcommand{\Gh}{\G[\Xh^+]}
\newcommand{\Ch}{\C_{\Gh}}
\newcommand{\ch}{c}
\renewcommand{\D}{\mathcal{D}}
\renewcommand{\M}{\mathtt{M}}
\newcommand{\mcc}{\textsc{Multi-Colored Clique} }
\newcommand{\srds}{$[\sigma,\rho]$-\textsc{Dominating Set} }
\newcommand{\jlds}{$[j,\ell]$-\textsc{Dominating Set} }
\newcommand{\1jds}{$[1,j]$-\textsc{Dominating Set}}
\newcommand{\Mi}{\M_\bli}
\newcommand{\Mj}{\M_\blj}
\newcommand{\Mh}{\M_\blh}
\renewcommand{\S}{\mathcal{S}}
\def\Si{\mathcal{S}_\bli}
\renewcommand{\Si}{\mathcal{S}_\bli}
\newcommand{\Sj}{\mathcal{S}_\blj}
\newcommand{\Sh}{\mathcal{S}_\blh}
\newcommand{\T}{\mathcal{T}}
\newcommand{\TD}{\mathtt{T}}
\newcommand{\X}{X}
\renewcommand{\Xi}{X_\bli}
\newcommand{\Xj}{X_\blj}
\newcommand{\Xh}{X_\blh}
\newcommand{\Xr}{X_\blr}
\newcommand{\tw}{\textbf{tw}}
\newcommand{\pw}{\textbf{pw}}

\newtheorem{observation}[theorem]{\textbf{Observation}}


==> fpttwk.tex <==
\section{A $(k+1)^{\tw(G)}$ algorithm for MMDS}
\label{apdx:xpAlgo}
In this section, we consider the MMDS problem parameterized by the treewidth of input graph and solution size $k$. 
To describe the algorithm, we first define the nice tree decomposition of a graph. 
A tree decomposition $(\T, \X)$ is said to be {\em nice} if $\T$ is rooted by a node $\blr$ with $\Xr = \emptyset$, and each node in $\T$ is one of the following four types of nodes.
\begin{enumerate}
\item {\sf Leaf node.} A node $\bli \in V(\T)$ with no child and $\Xi = \emptyset$. 
\item {\sf Introduce node.} A node $\bli \in V(\T)$ with a child $\blj$ such that $\Xi = \Xj \cup \{v\}$ for some $v \notin \Xj$.
\item {\sf Forget node.} A node $\bli \in V(\T)$ with a child $\blj$ such that $\Xi = \Xj \setminus \{v\}$ for some $v \in \Xj$. 
\item {\sf Join node.} A node $\bli \in V(\T)$ with two children $\blj$ and $\blh$ such that $\Xi = \Xj = \Xh$. 
\end{enumerate} 

%We use a nice tree decomposition of the input graph $\G$. 
Let $(\T, \X)$ be a nice tree decomposition of $G$ rooted by node $\blr$. 
For each node $i \in V(\T)$, we compute a table $\Mi$ indexed by a two-tuple which we refer to as a state. 
Let $\Si$ denote the set of all states associated with node $\bli$. 
For a state $s \in \Si$, the DP formulation gives a recursive definition of the table $\Mi[s]$. $\Mi[s]$ is a binary indicator that is set to one if and only if the MMDS problem on instance $(\Gi, k)$ with additional constraints  specified by the state $s$ has a feasible solution. 
A state at the node $\bli$ is a tuple 
$(c,d)$,
%$(c:\Xi \to \{0,1\}, d:\Xi \to [0,k])$, 
where  %$c:\Xi \to \{0,1\}$ and $d:\Xi \to [0,k]$ be a pair of functions such that for each $u \in \Xi$,
\begin{itemize}
\item $c:\Xi \to \{0,1\}$ is an indicator function for $\Xi$ such that for each $u \in \Xi$, $c(u)$ indicates whether $u$ is included in the solution, and
\item $d:\Xi \to [0,k]$ is a function such that for each $u \in \Xi$, $d(u)$ is the membership of $u$ in the desired solution. 
\end{itemize}
If there is no feasible solution for the state $s$, then $\Mi[s]$ is set to zero. Also, we call the state $s$ as {\em invalid} state. 


\noindent {\bf State induced by a set at node $i$. }
For a set $S \subseteq \Xi^+$ of $\Gi$, we say that $S$ {\em induces} the functions $c:\Xi\to\{0,1\}$ and $d:\Xi\to[0,k]$ for the node $\bli$ such that for each $u \in \Xi$, $$c(u) = \begin{cases} 1 & \text{ if } u \in S,\\ 0 & \text{ otherwise}\end{cases}$$ and $d(u) = N[u] \cap S$. 
%The table entry $\Mi[c,d]$ is a binary value set to one if and only if there exists a set $S \subseteq \Xi^+$ such that $S$ induces $c$ and $d$. 

\noindent {\bf Correctness invariant.} For a pair of functions $c:\Xi\to\{0,1\}$ and $d:\Xi\to[0,k]$ of a node $\bli$, we will maintain:
\[\Mi[c,d] = \begin{cases} 1 & \text{ if there exists a set $S \subseteq \Xi^+$ such that $S$ induces $c$ and $d$},\\
0 & \text{ otherwise.} \end{cases}\]
From the root node $\blr$, we can find whether there exists a solution for the MMDS problem on instance $(G,k)$. 
Formally, at the root node $\blr$, the table entry $\Mi[c:\emptyset\to\{0,1\},d:\emptyset\to[0,k]]$ decides the existence of solution for the instance MMDS$(G,k)$. 

\subsection{Dynamic programming}
For each node $\bli \in V(\T)$, we show how to populate the table $\Mi$ from the populated table(tables) for the child(children) of $\bli$. 
Let $\bli$ be a node in $\T$, and $s = (c:\Xi \to \{0,1\}, d:\Xi \to [0,k])$ be a state at node $\bli$. % defined on $\Xi$.
We describe the computation of the table entry $\Mi[s]$ in cases according to the types of nodes of the
nice tree decomposition.

\noindent {\bf Leaf node.} Let $\bli$ be a leaf node with $\Xi = \emptyset$. 
We have one row in the table $\Mi$.
Let $s= (c:\emptyset \to \{0,1\}, d:\emptyset\to[0,k])$ be the state corresponding to the row and the table entry is given as $\Mi[s] = 1$. 
\begin{lemma}
\label{lem:leaf}
The table entry $\Mi[s]$ is updated correctly. 
\end{lemma}
Given the state $s$, we can compute the entry $\Mi[s]$ in time $O(1)$. 
Therefore:
\begin{observation}
\label{obs:leaf}
The time to compute the table $\Mi$ for a leaf node $\bli$ is $O\big((2k+2)^{n_\bli}\big)$
\end{observation}
\noindent {\bf Introduce node.} Let $\bli$ be an introduce node with only child $\blj$ such that $\Xi = \Xj \cup \{v\}$ for some $v \notin \Xj$. 
Let $A_1 = c\inv(1) \cap N[v]$. 
If $|A_1| \not= d(v)$, then the state $s$ has no feasible solution. 
Then $s$ is invalid and $\Mi[s] = 0$. 
Therefore, we consider $|A_1| = d(v)$. 
We define the state $s_\blj = (c_\blj:\Xj \to \{0,1\}, d_\blj:\Xj \to [0,k])$ and define $\Mi[s]$ in terms of $\Mj[s_\blj]$. 
We consider two cases that $c(v) = 0$ and $c(v) = 1$ to define the state $s_\blj$. 
\begin{itemize}
\item Case when $c(v) = 0$. For each $u \in \Xj$, $c_\blj(u) = c(u)$ and $d_\blj(u) = d(u)$. 
\item Case when $c(v) = 1$. 
Let $A_v = N(v) \cap \Xi$. 
For each $u \in \Xj$, $c_\blj(u) = c(u)$ and
$$ d_\blj(u) = \begin{cases}d(u) - 1 & u \in A_v\\ d(u) & \text{ otherwise.}\end{cases}$$ 
\end{itemize}
%%%%First we consider the case that $c(v) = 0$.  
%%%%%If $|C_v| \not= d(v)$, then $\Mi[c,d] = 0$. 
%%%%%Suppose $|C_v| = d(v)$, then 
%%%%Let us define $c_\blj:\Xj \to \{0,1\}$ and $d_\blj:\Xj \to [0,k]$ such that for each $u \in \Xj$, $c_\blj(u) = c(u)$ and $d_\blj(u) = d(u)$. 
%%%%Then, the entry $\Mi[c,d]$ is computed as follows:
%%%%\begin{equation}\label{eq:1}
%%%% \Mi[c,d] = \begin{cases} 0 & \text{ if } |A_1| \not= d(v)\\ \Mj[c_\blj, d_\blj] & \text{ otherwise.}\end{cases}
%%%% \end{equation}
%%%%Now we consider the second case that $c(v) = 1$. 
%%%%Let $A_v = N(v) \cap \Xi$. 
%%%%Let us define $c_\blj:\Xj \to \{0,1\}$ and $d_\blj:\Xj \to [0,k]$ such that for each $u \in \Xj$, $c_\blj(u) = c(u)$ and
%%%%$$ d_\blj(u) = \begin{cases}d(u) - 1 & u \in A_v\\ d(u) & \text{ otherwise.}\end{cases}$$ 
The entry $\Mi[s]$ is computed as follows:
\begin{equation}\label{eq:2}
\Mi[s] = \Mj[s_\blj]
 \end{equation}
\begin{lemma}
\label{lem:introduce}
Consider the state $s_\blj$ defined as above. The table entry $\Mi[s]$ is one if and only if $\Mj[s_j]$ is one. 
\end{lemma}
\begin{proof}
First suppose $\Mi[s] = 1$ and let $S \subseteq \Xi^+$ be a feasible solution that is a witness to
this. 
Note that the set $S\setminus\{v\}$ induces the state $s_\blj$ at node $\blj$. 
Then, the set $S\setminus \{v\}$ witnesses the fact that $\Mj[s_\blj] = 1$. 
Conversely, $\Mj[s_\blj]=1$ and let $S'$ be the set that is a witness to this. 
We define $S = S' \cup \{v\}$ if $c(v)  =1$, and $S = S'$, otherwise. 
Note that the set $S$ induces the state $s$ at node $\bli$. 
Then, the set $S$ witnesses the fact that $\Mi[s_\blj] = 1$. 
%If $|A_1| \not= d(v)$, then the vertex $v$ can not satisfied the membership constraint in any solution since $N[v] \cap \Xi^+ \subseteq \Xi$. 
%Therefore, the state $s$ is invalid. 
\qed\end{proof}
For a given functions $c$ and $d$, we can compute the entry $\Mi[c,d]$ in time $O(1)$. 
Therefore: 
\begin{observation}
\label{obs:introduce}
The time to compute the table $\Mi$ for an introduce node $\bli$ is $O\big((2k)^{n_\bli}\big)$
\end{observation}

\noindent {\bf Forget node.} Let $\bli$ be a forget node with only child $\blj$ such that $\Xi = \Xj \setminus \{v\}$ for some $v \in \Xj$. 
For each $a \in \{0,1\}$ and $b \in [1,k]$, let us define $s_\blj^{a,b} = (c_\blj^a:\Xj \to \{0,1\}, d_\blj^b:\Xj \to [0,k])$ such that for each $u \in \Xj$, \\
\begin{minipage}[t]{0.45\textwidth}
$$c_\blj^a = \begin{cases} a & \text{ if } u = v, \\c(u) & \text{ otherwise,}\end{cases}$$ 
\end{minipage}
\begin{minipage}[t]{0.45\textwidth}
$$ d_\blj^b = \begin{cases} b & \text{ if } u = v, \\d(u) & \text{ otherwise.}\end{cases}$$
\end{minipage}
%let us define $c_\blj^a:\Xj \to \{0,1\}$ such that for each $u \in \Xj$, 
%
%For each $b \in [1,k]$, let us define $d_\blj^b:\Xj \to [0,k]$ such that for each $u \in \Xj$, 

\noindent Note that we are not considered the case that $b=0$, because $b=0$ leaves the vertex $v$ is not dominated. 
Then, the table entry $\Mi[s]$ is computed as follows:
\begin{equation} \label{eq:3}
\Mi[s] = \displaystyle\bigvee_{\substack{a \in \{0,1\},\\ b \in [1,k]}} \Mj[s_\blj^{a,b}].
\end{equation} 
\begin{lemma}
\label{lem:forget}
There exists an $a \in \{0,1\}$ and $b \in [1,k]$ such that the table entry $\Mi[s]$ is one if and only if $\Mj[s_\blj^{a,b}]$ is one. 
\end{lemma}
\begin{proof}
First suppose $\Mi[s] = 1$ and let $S \subseteq \Xi^+$ be a feasible solution that is a witness to
this. 
Let $s_\blj = (c_\blj:\Xj \to \{0,1\}, d_\blj:\Xj \to [0,k])$ be the state induced by the set $S$ at node $\blj$. 
The vertex $v$ has $d_\blj(v) \geq 1$ since $v$ should be dominated by the set $S$. 
Note that the state $s_\blj$ is same as $s_{\blj}^{c_{blj}(v),d_\blj(v)}$. 
Then, the set $S$ witnesses that $\Mj[s_\blj] = 1$. 
Conversely, there exists $a \in \{0,1\}$ and $b \in [1,k]$ such that $\Mj[s^{a,b}_\blj] = 1$ and let $S$ be a set that is witness to this. 
Observe that the functions $c$ and $d$ are identical to $c_\blj^{a,b}$ and $d^{a,b}_\blj$ except for the vertex $v$. 
Therefore, the set $S$ is inducing the state $s$ and $S$ witnesses the fact that $\Mi[s] = 1$.
\qed\end{proof}
For a given state $s$, we can compute the entry $\Mi[s]$ in time $O(k)$. 
Therefore: 
\begin{observation}
\label{obs:forget}
The time to compute the table $\Mi$ for a forget node $\bli$ is $O\big((2k+2)^{n_\bli}k\big)$
\end{observation}
\noindent {\bf Join node.} Let $\bli$ be a join node with children $\blj$ and $\blh$ such that $\Xi = \Xj = \Xh$. 
For each vertex $u \in \Xi$, let $\ell_u = d(u) - |N[u] \cap c\inv(1)|$. 
For each function $g:\Xi \to [0,k]$ such that for each $u \in \Xi$, $0 \leq g(u) \leq \ell_u$, we define the states $s_\blj = (c, d_\blj^g :\Xj \to [0,k])$ and $s_\blh = (c, d_\blh^g:\Xh\to[0,k])$ such that for each $u \in \Xi$, 
$d_\blj^g(u) = |N[u] \cap c\inv(1)| + g(u)$
and 
$ d_\blh^g(u) = d(u) - g(u) $.
Then, the table entry $\Mi[s]$ is computed as follows:
\begin{equation}\label{eq:4}
\Mi[s] = \bigvee_{g:\Xi \to [0,k] \big| \forall u \in \Xi, 0 \leq g(u) \leq \ell_u } \Mj[s_\blj^g]\cdot\Mh[s_\blh^g]
\end{equation}
\begin{lemma}
\label{lem:join}
There exists a function $g:\Xi\to[0,k]$ such that the table entry $\Mi[s]$ is one if and only if both $\Mj[s_\blj^g]$ and $\Mh[s_\blh^g]$ are one. 
\end{lemma}
\begin{proof}
First suppose $\Mi[s] = 1$ and let $S \subseteq \Xi^+$ be a feasible solution that is a witness to
this. 
Let $S_{\blj} = S \cap \Xj^+$ and $S_\blh = S \cap \Xh^+$. 
Let $s_\blj = (c, d_\blj:\Xj \to [0,k])$ and $s_\blh = (c, d_\blh:\Xh \to [0,k])$ be the states induced by the sets $S_blj$ and $S_\blh$ at the nodes $\blj$ and $\blh$, respectively. 
Note that the states $s_\blj$ and $s_\blh$ are induced with function $c$ in common since $S \cap \Xi = S_\blj \cap \Xj = S_\blh \cap \Xh$. 
Let us define $g: \Xi \to [0,k]$ such that for each $u \in \Xi$, $g(u) = d_\blj(u) - |N[u] \cap c\inv(1)|$. 
Note that the states $s_\blj$ and $s_\blh$ are same as $s_\blj^g$ and $s_\blh^g$, respectively. 
Then, the sets $S_\blj$ and $S_\blh$ witness that $\Mj[s_\blj^g] = 1$ and $\Mh[s_\blh^g] = 1$, respectively. 
Conversely, there exists $g:\Xi \to [0,k]$ such that both $\Mj[s_\blj^g] = 1$ and $\Mh[s_\blh^g] = 1$. 
Let $S_\blj$ and $S_\blh$ be the sets that are witness to $s_\blj^g$ and $s_\blh^g$, respectively.
Let $S = S_\blj \cup S_\blh$. 
For each vertex $u \in \Xi$, $u$ has membership values $d_\blj^g(u)$ in $S_\blj$ and $d_\blh^g(u)$ in $S_\blh$. 
Moreover, the vertex $u$ is accounted for the membership value $|N[u] \cap c\inv(1)|$ in both sets $S_\blj$ and $S_\blh$. 
Therefore, the membership of $u$ in $S$ is 
\begin{eqnarray*}
M(u,S) &=& d_\blj^g(u) + d_\blh^g(u) - |N[u] \cap c\inv(1)| \\
&=& |N[u] \cap c\inv(1)| + g(u) + d(u) - g(u) - |N[u] \cap c\inv(1)|\\
&=& d(u)
\end{eqnarray*}
The set $S$ induces the state $s$ since $S \cap \Xi = c\inv(1)$ and each vertex $u \in \Xi$ agrees the membership value constrained by the function $d$. 
Then, the set $S$ witnesses the fact that $\Mi[s] = 1$. 

 
Observe that the functions $c$ and $d$ are identical to $c_\blj^{a,b}$ and $d^{a,b}_\blj$ except for the vertex $v$. 
Therefore, the set $S$ is inducing the state $s$ and $S$ witnesses the fact that $\Mi[s] = 1$.
\qed\end{proof}
For a given state $s$, we can compute the entry $\Mi[s]$ in time $O((k+1)^{n_\bli})$. 
Therefore: 
\begin{observation}
\label{obs:join}
The time to compute the table $\Mi$ for a join node $\bli$ is $O\big((2(k+1)^2)^{n_\bli}\big)$
\end{observation}
In the following lemma we argue the correctness of  the table entries. 
\begin{lemma}
For each node $i \in V(\T)$, and for each state $S = (c:\Xi\to\{0,1\}, d:\Xi\to[0,k])$, the correctness invariant is maintained for $\Mi[s]$. 
\end{lemma}

\begin{proof}
The proof is by induction on the height of a node in $\T$. 
Recall, that the height of a node $\bli$ in the rooted tree $\T$ is the distance to the furthest leaf in the subtree rooted at $\bli$. 
The base case is when $\bli$ is a leaf node $\T$ and height is 0 and the proof of the claim follows from Lemma~\ref{lem:leaf}.
Let us assume that the claim is true for all nodes in $\T$ of height at most $h-1 \geq 0$. 
We now prove that if the claim is true for all nodes of height at most $h-1$, then it is true for a node of height $h$. 
Let $\bli$ be a node of height $h \geq 1$. 
Since $\bli$ is not a leaf node, its children are at height at most $h-1$. 
Therefore, by the induction hypothesis, the correctness invariant is maintained at all the
children of $\bli$. 
Now, we prove that the correctness invariant is maintained at node $\bli$. 
Let $s$ be a state in node $\bli$. 

If $\bli$ is an introduce node then from Lemma~\ref{lem:introduce}, we know that the state $s$ in $\bli$ is valid if and only if the state $s_\blj$ at node $\blj$ is valid. 
Similarly, if $\bli$ is a forget node, then from Lemma~\ref{lem:forget} we know that the state $s$ in $\bli$ is valid if and only if there exists $a \in \{0,1\}$ and $b\in[1,k]$ such that the state $s_\blj = s_{\blj}^{a,b}$ at node $\blj$ is valid. 
By the induction hypothesis in both these cases the correctness invariant maintained in $\Mj[s_\blj]$ proves that the correctness invariant is maintained in $\Mi[s]$. 
If $\bli$ is a join node then from Lemma~\ref{lem:join}, we know that the state $s$ in $\bli$ is valid if and only if there exists function $g:\Xi \to [0,k]$ such that the states $s_\blj = (c, d_\blj^g)$ and $s_\blh = (c, d_\blh)$ are valid at the nodes $\blj$ and $\blh$, respectively. 
Therefore, it follows from the induction hypothesis that the correctness invariant maintained in $\Mj[s_\blj^g]$ and $\Mh[s_\blh^g]$ proves that the correctness invariant is maintained in $\Mi[s]$. 
This completes the proof.
%%%%\noindent {\bf Case 1 : $\bli$ is an Introduce node -} Let $\blj$ be the only child of $\bli$, where $\Xi = \Xj \cup \{v\}$ for some $v \notin \Xj$. 
%%%%We consider the cases when $c(v) = 0$ and $c(v) = 1$. % separately for which the table entry updations are indicated by \ref{eq:1} and \ref{eq:2} respectively.  The correctness of \ref{eq:1} is justified by the fact that if we assign value 0 to
%%%%First we consider the case that $c(v)=0$. That is the vertex $v$ is not part of  then $v$ is not part of the solution and we only need to check whether the $d$ value of $v $, which implies the number of times vertex $v$ gets dominated, is equal to the number of neighbors of $v$ whose $c$ value is 1, ie, $|N[v]\cap c\inv (1)|$.
%%%%
%%%% Now, when $c(v) = 1$, $\forall u \in N[v]\cap \Xi~~ d_\blj(u) = d(u)$-1. This is true, since the number of dominations for the neighbors of $v$ would have incremented in $\Xi$ by the introduction of vertex $v$. Similar to above case, we need to check if $d(v) = |N[v]\cap c\inv (1)|$ as a safety condition.\\
%%%%
%%%%
%%%%\noindent {\bf Case 2 : $\bli$ is a Forget node -} Let $\blj$ be the only child of $\bli$, where $\Xi = \Xj \setminus \{v\}$ for some $v \in \Xj$. $c$ and $d$ values of forgotten vertex $v$ in $\Xj$ could have been any combination and we need to check for all possibilities, If any of those table entries in $\Mj$ happens to be valid, $\Mi[c.d]$ is made valid. This justifies the correctness of Equation \ref{eq:3}.\\ 
%%%%
%%%%\noindent {\bf Case 3 : $\bli$ is a Join node -} Let $\blj$ and $\blh$ be the children of node $\bli$ such that $\Xi = \Xj = \Xh$. We first compute a value $\ell_u $ for each $u\in \Xi$ where $\ell_u $ is the remaining number of dominations for vertex $u$, other than what is contributed by $N[u]\cap c\inv(1)$. Now, $\ell_u $ many dominations for vertex $u\in \Xi$ should come from $ N[u]\cap c_{\blj}\inv(1)$ and $N[u]\cap c_{\blh}\inv(1)$. All possible combinations are to be checked and $\Mi[c.d]$ is made valid accordingly. Equation  \ref{eq:4} specifies the above operation.\\
%%%%
%%%% This completes the proof  for node $\bli$ being different types of nodes in the given nice tree decomposition $(\T, \X)$. 
%%%%
%%%%For any node $\Xi$, for every $(c',d')\in \Mi\inv(1)$ we claim that 
%%%%\begin{equation*}
%%%%p \leq k, ~\forall p\in d'.
%%%%\end{equation*}
%%%%i.e,  the current maximum number of times any vertex is dominated is always less than or equal to $k$ in any valid table entry. The function $d$ is defined only for $\Xi \to  [0,k]$ and it is checked while updating the table.
%%%%
%%%%The solution(s) for the given MMDS instance can be obtained from the valid entry/entries in the table for the root node $\T$.
 \qed\end{proof}
 
Finally, from Observations~\ref{obs:leaf},~\ref{obs:introduce},~\ref{obs:forget}~and~\ref{obs:join}, For each node $\bli \in V(\T)$, the table $\Mi$ can be populated in $O((2(k+1)^2)^{\tw(G)})$ time. 
A nice tree decomposition with $O(n\cdot w)$ can be obtained in polynomial time\cite{Kloks94}. 
Thus, the algorithm runs in time $O((2(k+1)^2)^{\tw(G)})n^{O(1)}$
%Therefore, the Lemma~\ref{lem:treewidth} completes the proof of Theorem~\ref{thm:treewidthK}. 


==> intervalgreedy.tex <==
In this section we study the \mmds problem for interval graphs. Recall that interval graphs are graphs consisting of a set of intervals along the real line, with a vertex for each interval and an edge between vertices whose intervals intersect. 

\subsection{3-mds for Interval graphs}
We show that for any interval graph, a solution to the $k$-MMDS problem can be found by a polynomial time greedy algorithm when $k\geq 3$. Algorithm\ref{alg:Algo1} describes how to do the same. We consider the input to be the interval representation of the graph. Let $\mathcal{I}$ be the set of intervals given. We run the greedy algorithm starting with the interval with leftmost left endpoint. If there is a tie, select the larger interval (hence the one whose right endpoint is to the right of the others in tie). Let this interval be $I$ and its left and right endpoints be $l(I)$ and $r(I)$ respectively. We build the solution set $S$ by adding $I$ to $S$. $I$ dominates all intervals overlapping with it. Next, we select the interval with the rightmost right endpoint among the intervals which crosses $r(I)$. Let this be $I'$ and note that it is dominated by $I$. Now $I'$ becomes the new $I$ and gets added to the solution set $S$. The algorithm continues until there are no more intervals left to be dominated.\\

 \SetNlSty{texttt}{(}{)}
\begin{algorithm}

    \SetAlgoLined
    $Q \gets \mathcal{I}$;\\
    Let $I$  be  the interval with leftmost left endpoint ;\\
    $l(I)$ = left endpoint  of $I$;\\
	$r(I)$ = right endpoint of $I$;\\
 \While{$Q\neq\emptyset$ }
     {
	
	$S\gets I$;\\
	$I'\gets  $ Interval which crosses $r(I)$ and with right most right endpoint;\\
	$Q'\gets \{$ intervals overlapping with $I\}\setminus I'$;\\
	$Q\gets Q\setminus Q'$;\\
	$I\gets I'$;\\
 }
 Output $S$;\\
    \caption{\mmds Greedy algorithm for intervals  }
  \label{alg:Algo1}
 
 \end{algorithm}
 \input{bigpic.tex}
 \begin{lemma}
  The output of \textbf{Algorithm\ref{alg:Algo1}} gives a dominating set for the given set of intervals $\mathcal{I}$. 
 \end{lemma}
 \begin{proof}
 We use the method of proof by contradiction. Assume that the output set $S$ of the algorithm does not form a dominating set. i.e, there is an interval $I''$ which is not dominated by $S$. From the description of the algorithm, it is clear that $S$ induces  a path in $\mathcal{I}$. Now we check the position of $I''$. It cannot be before the starting of the path $S$, as $S$ contains the leftmost interval. $I''$ cannot be placed in a point inside path $S$ since it will get dominated by at least one interval $I'\in S$ where $I'\cap I''\neq \emptyset$. Similarly, $I''$ cannot be to the right of $S$, since $S$ has the interval with rightmost right endpoint. This indicates, there is no such $I''$ which not dominated by $S$. Therefore $S$ is a dominating set for $\mathcal{I}$.
\qed \end{proof}
\begin{proof}[{\bf Proof of Theorem \ref{thm:intervalupperbound}}] 
Here we prove that $\forall I\in \mathcal{I},~~ M(I, S)\leq 3$, where $M(I, S)$ demotes the membership of $I$ in $S$. The proof is by contradiction. Assume that there is an $I\in \mathcal{I}$ such that  $M(I, S) > 3$.  Let the intervals intersecting with $I$ in $S$ be $I_i, I_{i+1}, I_{i+2}, \dots, I_j$, where $j > i+2$. $l(I)\leq r(I_i)$, because of the intersection between $I$ and $I_i$. Similarly $r(I) > r(I_i)$, since $I$ is intersecting with $ I_{i+2}$ and $l(I_{i+2}) > r(I_i)$ by the selection of $I_i$ and $I_{i+2}$ to $S$. By the algorithm, of all the intervals crossing $r(I_i)$, $I_{i+1}$ has the largest right endpoint. i.e, $r(I) < r(I_{i+1})$. Since $I$ intersects with $I_{i+2}$  as well, $l(I_{i+2}) \leq r(I_i)$. This leads to $l(I_{i+3}) \leq r(I_i)$ because of the intersection between $I$ and $I_{i+3}$. But this cannot happen as $l(I_{i+3})  > r(I_{i+1})$ by construction of $S$ and $r(I) < r(I_{i+1})$.  Therefore, this is a contradiction to the assumption that $M(I, S) > 3$.
\qed\end{proof}

\subsection{1-DS (Exact Dominating Set) and 2-DS of Interval Graphs}
Let $G=(V,E)$ be the given interval graph. An exact dominating set of a graph is a set $D\subseteq v$ such that for every $v\in V,~ N[v]\cap D = 1$. Thus exact dominating set is a special case of \textsc{MMDS} in which $k = 1$. We prove that exact dominating set of interval graphs can be found in polynomial time by a dynamic programming algorithm.\\

\noindent Let $C_1, C_2,\dots, C_r$ be the linear ordering of the maximal cliques of $G$. It is clear that the solution set $D$ contains a vertex $u\in C_1$. If there is no such vertex, the vertices occuring only in $C_1$, for $C_1$ being a maximal clique, will be left undominated. Let the rightmost maximal clique which contains $u$ be $R(u)$. Without loss of generality, let us assume that $R(u)$ is nonempty, since otherwise we are done with $u$ dominating everything. Now consider $u'\in R(u)$ such that $u'$ is a neighbor of $u$ and has the rightmost right endpoint. We define $A(u) = \{v~\mid~ v \text{ starts after $u$ and before $u'$ ends}\}$. 


\begin{figure}
\centering
\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
\draw(3,2)--(8,2);
\draw(8,0.5)--(12,0.5);
\draw (8.7,1.5)--(9.7,1.5);
\draw(10.2,1.5)--(11.2,1.5);
\draw (12,1.7)--(14,1.7);

\draw (3,1) ellipse (0.5cm and 1.75cm);
\draw (5,1) ellipse (0.5cm and 1.75cm);
\draw[dotted] (6,1)--(7,1);
\draw (8,1) ellipse (0.5cm and 1.75cm);
\draw[dotted] (9,1)--(11,1);
\draw (12,1) ellipse (0.5cm and 1.75cm);
\draw (14,1) ellipse (0.5cm and 1.75cm);
\draw[dotted] (15,1)--(16,1);
\draw (17,1) ellipse (0.5cm and 1.75cm);


\draw(3,-1) node{$C_1$};
\draw(8,-1) node{$R(u)$};

\draw(12,-1) node{$C_X$};
\draw(14,-1) node{$C_{X+1}$};
\draw(17,-1) node{$C_r$};
\draw(6,2.2) node{$u$};
\draw(10,0.3) node{$u'$};
\draw(9.2,1.7) node{$v_1$};
\draw(10.7,1.7) node{$v_2$};

%\draw(5,-1) node{$z_m$};
%\draw(7,-1) node{$z_t$};
%\draw(8,-0.75) node{$r'$};
%\draw(9,-0.75) node{$r'+1$};
\end{tikzpicture}
\label{fig:ProofFig2}
\caption{Example showing linear maximal clique ordering}
\end{figure}

\begin{observation}
 If $u\in D ,~ A(u)=\emptyset$.
\end{observation}
\begin{proof}
 Let there be a  vertex $v\in A(u)$. Note that $A(u)\cap D = \emptyset$ and $u'\notin D$, as $u'$ is already dominated by $u$ and will get dominated more than once if any vertex from $A(u)$ or $u'$ itself is selected to the solution set $D$.  Therefore the vertex $v$ will not be dominated by any of its neighbours, contradicting the fact that $D$ is a dominating set.
\end{proof} 
  
$$D(u, 1, r) = \bigg[\bigvee_{v\in C_{X+1}}D(v, X+1, r)\bigg]\bigwedge \bigg(A(u)= \emptyset\bigg)$$  

\noindent Hence there is an optimal substructure property to the 1-\textsc{MMDS} or Exact Dominating Set problem.



==> introduction.tex <==
\section{Introduction}
For an undirected graph $G=(V,E)$, a {\em dominating set} of $G$ is a set of vertices $S$ such that every vertex of $G$ is either in $S$ or has a neighbor in $S$. 
Computing a minimum  cardinality dominating set of a given graph $G$ is a classic $\NP$-hard problem~\cite{GareyJohnson79}. 
%The parameterized dominating set problem has been studied extensively. 
%We refer the reader to the books~\cite{HaynesHS98:2,HaynesHS98} by Haynes, Hedetniemi and Slater for more information about the minimum dominating set problem and its applications. 
Further, there are studies on dominating sets with constraints on the cardinality of the intersection between the closed neighborhood of a vertex and the dominating set.  
In this paper we study dominating sets under one such constraint, which we refer to as \emph{Minimum Membership Dominating Set }(\textsc{MMDS}). 
We adapt the definition of {\em membership} from Kuhn \textit{et al.}~\cite{KuhnRWWZ05} where the authors defined it for a set system. 
Given a vertex $u$ and a vertex subset $S$, the membership of $u$ in $S$ is denoted by $M(u, S) = |N[u] \cap S|$.
Throughout this paper, when we use the phrase {\em membership of a vertex $u$}, we mean membership of $u$ in $S$.
%the membership of a vertex $u$ is with respect to a set of vertices $S$.
%\begin{definition}[Kuhn \textit{et al.}~\cite{KuhnRWWZ05}]
%Given a vertex $u \in V$ and a set $S\subseteq V$, the {\em membership} of $u$ in $S$, denoted by $M(u,S) = |N[u] \cap S|$. 
%\end{definition}
Given an input graph $G=(V,E)$, the MMDS problem asks to find a dominating set $S$ such that the maximum membership of any vertex is minimized. 
The parameterized version of the MMDS problem is defined as follows.
\begin{tcolorbox}

\textbf{Minimum Membership Dominating Set (MMDS)}\\
\textbf{Input}: A graph $G=(V, E)$ and a positive integer $k$\\
\textbf{Parameter:} $k$\\
\textbf{Question}: Does there exist a dominating set $S$ of $G$ such that $\max_{u\in V}M(u, S) \leq k$?
\end{tcolorbox}

\noindent\textbf{Membership: }
The term \emph{membership} was introduced by Kuhn \textit{et al.}~\cite{KuhnRWWZ05} in their paper on \emph{Minimum Membership Set Cover} (\textsc{MMSC}). 
In the \textsc{MMSC} problem, given a set system $\mathcal{X} = (S, C)$, where $S$ is a set of elements and $C \subseteq 2^{\{S\}}$, the aim is to find a subset $C'\subseteq C$ which  covers all elements in $S$ such that each element in $S$ occurs at most $k$ times in $C'$. 
The \textsc{MMSC} problem was devised as a measure to reduce interference among transmitting base stations in cellular networks. 
The idea is to control the power of transmission for each base station such that the number of base stations covering any client is minimum while ensuring that each client is covered by at least one base station. 
This is modeled by  a set system $\mathcal{X} = (S, C)$ where $S$ denotes the set of clients  and each subset in $C$ denotes the clients covered by a particular base station. Kuhn \textit{et al.}~\cite{KuhnRWWZ05} showed that the \textsc{MMSC} problem is  $\NP$-complete by a reduction from Minimum Set Cover problem. 
They gave an $\mathcal{O}(\ln n)$ approximation algorithm for the \textsc{MMSC} problem and showed that there is no polynomial time approximation algorithm with ratio better than $\mathcal{O}(\ln n)$ unless $\NP \subset TIME(n^{O(\log \log n)})$. 
A special case of the \textsc{MMSC} problem is studied in~\cite{DomGNW06} where the collection of sets have \emph{consecutive ones property}. 
In such a set system, the problem is shown to be polynomial time solvable.  
Narayanaswamy \textit{et al.}~\cite{DhannyaNR18} and recently, Mitchell and Pandit~\cite{MitchellPandit19} have studied the dual of the \textsc{MMSC} problem which is the \emph{Minimum Membership Hitting Set} (\textsc{MMHS}) problem in various geometric settings. 
%Let $(U,X)$ be a set system where $U$ is a universe of elements and $X$ is a set of subsets of $U$. A hitting set $S\subseteq U$ is as set which intersects with every $x_i \in X$, that is $S$ is said to hit each $x_i \in X$.
% Minimum membership version of the hitting set problem (\textsc{MMHS}) tries to find a hitting set while minimizing the number of times each $x_i\in X$ is hit. Narayanaswamy \textit{et al.}~\cite{DhannyaNR18} showed that the \textsc{MMHS} problem does not admit a $2 - \epsilon$  approximation even in geometric settings like vertical line segments are hit by horizontal line segments. A polynomial time algorithm was given for the case when the horizontal segments are intersected by vertical lines.  Recently,  Mitchell and Pandit~\cite{MitchellPandit19}  studied both the \textsc{MMSC}  problem and the \textsc{MMHS} problem on various types of geometric objects in the plane, including axis-parallel line segments, axis-parallel strips, rectangles that are anchored on a horizontal line from one side, rectangles that are stabbed by a horizontal line, and rectangles that are anchored on one of two horizontal lines. For each of these problems, they either proved the $\NP$-hardness or gave a polynomial time algorithm.
%{\bf mostly this paragraph can be removed. All the points below are covered}
%\noindent The {\sc Dominating Set} problem is closely related to the {\sc Set Cover} problem. In fact the two problems are equivalent using the $L$-reduction~\cite{articlePhdThesis}. Minimum Set Cover (MSC) problem is proved to be W[2]-hard with respect to the parameter 'solution size'~\cite{DBLP:series/mcs/DowneyF99, DBLP:books/ox/Niedermeier06}. Similarly, Minimum Dominating Set is proved to be W[2]-Complete~\cite{DBLP:journals/siamcomp/DowneyF95}. However, a study of the membership version in parameterized setting has not been done to the best of our knowledge. In this paper, we look at the problem of finding a dominating set, while minimizing the number of times each vertex gets dominated. We study the problem of Minimum Membership Dominating Set in the parameterized setting.
%\subsection{Our Results}
%We show that \sf{MMDS} is $\NP$-Complete even for $k=1$. Therefore the solution size cannot be taken as a parameter for finding a parameterized solution. It is shown that \sf{MMDS} is W[1]-hard with treewidth as the parameter by  a reduction from {\sc Multicolored Clique} problem which is known to be W[1]-hard for the parameter $k$, the solution size. We give an FPT algorithm for \sf{MMDS} using the combined parameter treewidth and solution size ie, with parameter $(tw, k)$.

\noindent
%\subsection{Our contribution}
{\bf Our Results.}
%In contrast to dominating set problem where $k$ is the sthe parameter solution size ($k$) for the dominating set problem, the membership upper bound ($k$) is the natural parameter for the MMDS problem. 
The MMDS problem is a natural graph theoretic variant of the MMHS problem.
A natural question is whether the MMDS problem is FPT with respect to membership as the parameter.  We emphasize that here we have no restriction on the size of the dominating set, and aim to only optimize the membership.   
In the rest of the article, the membership parameter is denoted by $k$.
%the parameter $k$ where $k$ is the membership parameter. 
%We  show that the MMDS problem is \NP-complete restricted to planar bipartite graphs  for $k=1$. 
%\begin{theorem}
%\label{thm:planarhard}
%The MMDS problem is \NP-complete on planar bipartite graphs for $k=1$. 
%\end{theorem}
%This shows that the MMDS problem for the parameter $k$ is \texttt{Para}-{\tt NP}-hard, even for planar bipartite graphs.
%In other words, for every polynomial time computable function $f$, there is no $O(n^{f(k)})$-time algorithm for the MMDS problem. Further, our reduction also shows that the MMDS restricted to planar bipartite graphs does not have a $(2-\epsilon)$ approximation for any $\epsilon > 0$.  
 
%\textcolor{red}
%{However, this is not surprising as the problem has the flavor of the exact cover or exact hitting set problem~\cite{DhannyaNR18}. 
%Further, dominating set is also hard even when restricted to planar bipartite graphs.  
%On the other hand, for the minimum dominating set problem on planar graphs,  it is well known that Baker's technique gives a PTAS~\cite{Baker94}. 
%In our initial attempts, we were unable to make the Baker's technique work to give any approximation to the MMDS problem on planar graphs.    
%Thus even in planar graphs the MMDS with respect to membership as the parameter  is very different from the case of the minimum dominating set~\cite{AlberBFKN02}. 
One of the natural questions is whether MMDS is FPT by dynamic programming on a tree decomposition.  
%This is also a crucial sub-routine in the Baker's technique for many problems.   
We address the complexity of the MMDS problem with respect to treewidth as the parameter. To the best of our knowledge we do not know of any previous work on this problem. The attempts which are most similar to our work are for restricted cases of the \srds problem by Chapelle~\cite{Chapelle10} (which follow in our survey of previous work). 
We prove the following hardness result.
\begin{theorem}
\label{thm:twhard}
The MMDS problem is W[1]-hard with respect to pathwidth of the input graph as the parameter.
\end{theorem}
Our reduction is a gadget-based reduction from the \mcc problem which is known to be W[1]-complete. Thus, all the hardness results known for \mcc in the parameterized setting carry over to the MMDS problem parameterized by pathwidth.  Thus the MMDS is very different from minimum dominating set with respect to pathwidth.
% Multicolored Clique. 
%In particular, we show that an instance of the \mcc problem has a $k$-clique if and only if the reduced instance has a dominating set of membership at most $n+1$ where $n$ is the number of vertices in each partition. 
%Further, our reduction guarantees that the reduced instance has a pathwidth of at most $4 {k \choose 2} + 5$. 
%As a consequence of this reduction, we transfer all the hardness results known for the \mcc problem with parameter $k$ to the MMDS problem with $\pw(G)$ as the parameter. 
%More precisely, under the exponential time hypothesis it cannot be solved in $n^{o(\pw(G))}$ time. 

We observe that there is a $k^{\tw(G)}$ algorithm for the the MMDS problem. This algorithm is described in
  Theorem~2 of Chapelle~\cite{Chapelle10} for the  \srds problem and we obtained our algorithm for MMDS by invoking their algorithm with $\sigma = [0,k-1]$ and $\rho=[1,k]$.
%gives an XP algorithm for the MMDS problem for the parameter $\tw(G)$. 
The algorithm is a natural dynamic programming on a nice tree decomposition of the given graph. \\
%For the sake of completeness we state this as the following theorem, we present the detailed algorithm in the full paper in the Appendix.
%We complement the hardness result by showing a time $(2k+2)^{O(\tw(G))}n^{O(1)}$ algorithm on graphs of treewidth $w$. 
%\begin{theorem}
%\label{thm:combfpt}
%The MMDS problem admits an $O(k^{\tw(G)}n^{O(1)})$ algorithm with respect to membership $k$ and treewidth of the input graph as a combined parameter.
%\end{theorem}

Further, we analyze MMDS for split graphs and with respect to vertex cover.
Split graphs are graphs whose vertices can be partitioned into a clique and an independent set.
 
\begin{theorem}
\label{thm:splitreduction}
The \mmds problem is \textsc{W}[1]-hard for split graphs when parameterized by the size of membership.
\end{theorem}

We prove the above theorem by a reduction from \mcis problem. While \textsc{Dominating Set} is \textsc{W}[2]-hard on split graphs as well, recall that \mmds does not require optimizing the size of the solution size. \\ 

\noindent A parameterized problem can be studied with respect to various parameters. While the solution size is a natural choice for a parameter for analysis of many problems, often problems are studied with respect to other parameters related to the input. In graph theory, when the complexity analysis of a problem is with respect to parameters that reflect structural details of the input graph, such a parameterization is referred to as structural parameterization. In this paper, we study the algorithmic complexity of \textsc{MMDS} with respect to the parameter size of a vertex cover. We give two results in this regard. 


\begin{theorem}
\label{thm:vcFPT}
\textsc{MMDS} is FPT when parameterized by the size of vertex cover.
\end{theorem}

It is worth noting that \textsc{Dominating Set} is also FPT when parameterized by the size of vertex cover.

\begin{theorem}
\label{thm:vclowerbound}
For a graph $G$ with vertex cover $VC(G)$, $|VC(G)|\geq 3$, there does not exist an algorithm running in time $2^{o(|VC(G)|)}poly(n) $ that solves \textsc{MMDS}, unless ETH fails.
\end{theorem}

%In the parameterized \emph{dominating set problem}, the input is a graph $G$ and a positive integer $k$, and the goal is to decide whether there is a dominating set of $G$ of size at most $k$. 

\noindent
{\bf Related works.} In parameterized complexity, the minimum dominating set problem is well-studied %~\cite{CyganFKLMPPS15,
%DowneyFellows99,
%DowneyFellows13,
%FlumGrohe06,
%Niedermeier06}, 
%with a hope that in practice we are mostly interested in graphs with smaller dominating sets.}
%\textcolor{blue}{ In that case, an algorithm which is single exponential in solution size can also be considered practically viable.} 
%However, the dominating set problem 
and it is W[2]-complete~\cite{DowneyFellows95}, and thus fixed parameter intractable unless FPT = W[2]. Further, it is FPT for planar graphs. Besides, with treewidth of the input graph as the parameter, the minimum dominating set problem is FPT~\cite{AlberBFKN02}.  Recently, Chen and Lin~\cite{ChenLin19} proved that any constant-approximation for the parameterized dominating set problem is W[1]-hard. 
%\textcolor{blue}{
%MMDS seeks a solution without restriction on the size but on the membership value. 
%Whereas, most of the variants of the dominating set problem are seeking a minimum size solution that satisfies some additional properties. 
%}
There are many results in the literature which consider a combination of membership and the size of the dominating set, which we outline below.

\noindent {\bf Perfect code.} \noindent A \emph{perfect dominating set} or a {\sc Perfect Code} of a graph $G=(V,E)$ is a subset $V'\subseteq V$ satisfying the conditions (i) $V'$ is a dominating set, and (ii) for each $v \in V$, $|N[v] \cap V'| = 1$, %(\st{$N[u]\cap N[v] = \emptyset$ for all $u,v \in V',~ u \neq v$}) 
where $N[u]$ denotes the closed neighborhood of vertex $u$.   
The {\sc Perfect Code} problem has been studied extensively~\cite{Biggs73,FellowsH91,HuangXZ18,Kratochvil86,Kratochvil87,Mollard11,CESATI2002}, and we observe that
it is a special case of the MMDS problem. That is, {\sc Perfect Code} of a graph $G$ and MMDS for $k=1$ are equivalent. 
Kratochvil and Krivanek~\cite{KratochvilK88} have shown that {\sc Perfect Code} is $\NP$-complete on 3-regular planar graphs. 
Further, the parameterized {\sc Perfect Code} problem is W[1]-hard when the size of dominating set is the parameter~\cite{DowneyFellows92}.  Subsequently, it was shown to be complete for W[1] by Cesati~\cite{CESATI2002}.  

%$k$-{\sc Perfect Code} is the parameterized version of the {\sc Perfect Code} that seeks a {\sc Perfect Code} of size at most $k$. Downey and Fellows has shown that $k$-{\sc Perfect-Code} is W[1]-hard when parameterized by $k$. 
\noindent {\bf [$\sigma,\rho$]-dominating set.} %Another variant of the dominating set different from the minimum cardinality dominating set is the \srds problem introduced by 
Telle~\cite{Telle94J,Telle94T} introduced a generalized dominating set called [$\sigma,\rho$]-{\sc Sominating Set}. 
Let $\sigma,\rho \subseteq \mathbb{N}$ be two sets of non-negative integers.
Given a graph $G=(V,E)$, the \srds problem seeks to decide if there exists a set $S \subseteq V$ such that for each $u \in S$, $|N(u) \cap S| \in \sigma$, and for each $u \notin S$, $|N(v) \cap S| \in \rho$.  Here $N(u)$ refers to the open neighborhood of $u$.
Notice that the sets $\sigma$ and $\rho$ are part of the definition of the problem and not part of an input instance. 
Chapelle~\cite{Chapelle10} showed that the \srds problem is FPT parameterized by the treewidth of the input graph, when the size of the sets $\sigma$ and $\rho$ are bounded by a constant. 
More precisely, there is a $(|\sigma| + |\rho|)^{\tw(G)}n^{O(1)}$ time algorithm to solve the \srds problem, where $\tw$ is the treewidth of the input graph.
%When  $\sigma$ contains arbitrarily large gaps between two consecutive elements and $\rho$ is cofinite, they showed that  the \srds problem is W[1]-hard for the parameter treewidth of the input graph.  The study of this variant of dominating set with respect to treewidth as the parameter is the common feature between our results on the MMDS, and the hardness known for \srds problem.
\noindent As a special case of \srds problem, the \jlds problem was introduced by Chellali \textit{et al.}~\cite{ChellaliHHM13}. For any two positive integers $j$ and $\ell$, a subset $D\subseteq V$ in a graph $G=(V,E)$ is a {\em $[j,\ell]$-set} if, for every vertex $v\in V\setminus D,j\leq|N(v)\cap D|\leq \ell$. 
That is, each vertex $v\in V\setminus D$ is adjacent to at least $j$ vertices, but not more than $\ell$ vertices in $D$. Thus the \jlds problem is a generalization of the minimum cardinality dominating set problem, since
%The MMDS problem is a special case of the \jlds problem with $j=1$ and $\ell = k$. 
for $j\geq 1$ and $\ell \geq \Delta(G)$, a $[j,\ell]$-set $D$ is a dominating set.
%since every vertex in $V\setminus D$ has at least one neighbor in $D$.  
The focus in  ~\cite{ChellaliHHM13} was on $[1,2]$-\textsc{Dominating set} and they observed that for any simple graph $G$, $\gamma(G)\leq \gamma_{(1,2)}(G)\leq n$. For claw-free graphs, $P_4$-free graphs, and caterpillars, it was shown that  $\gamma(G) = \gamma_{(1,2)}(G)$. 
%\textcolor{red}
A recent paper by Meybodi \textit{et al.}~\cite{MeybodiFMP20}, study the problems \rjds, $[1,j]$-\textsc{Total Dominating Set} and \textsc{Restrained Dominating Set} in a parameterized perspective.  A set $D\subseteq V(G)$ is called a $[1,j]$-Total Dominating Set if every vertex in $V(G)$ has at least one and at most $j$ neighbors in $D$. In $[1,j]$-\textsc{Total Dominating Set} problem, the aim is to check the existence of  a $[1,j]$-Total Dominating Set of size at most $k$, on input of a graph $G$ and a positive integer $k$. Given a graph $G$ and a positive integer $k$, the \textsc{Restrained Dominating Set} problem asks if there is a dominating set $D$ of $G$ of size at most $k$ such that no vertex outside of $D$ has all of its neighbors in $D$. %\rjds problem is proved to be W[1]-hard for $d$-degenerate graphs whereas it is FPT on nowhere dense graphs. They also prove that $[1,2]$-\textsc{Total Dominating Set} problem cannot be solved in $O^*(4-\epsilon)^{pw}$ assuming Strong Exponential Time Hypothesis, where $pw$ is the pathwidth of the given graph and  \textsc{Restrained Dominating Set} is W[1]-hard even on 3-degenerate graphs. 
A comparative study of these problems in parameterized perspective are given in Table \ref{tab:table1}.
In all these problems, the parameter $k$ refers to the cardinality of the solution set, whereas in the \textsc{MMDS} problem, $k$ refers to the membership. From the table it is clear that the parameterized complexity of the MMDS problem is a natural question in the light of the treewidth based hardness results for the constrained variants of the $[\sigma,\rho]$-Dominating set problem.  To the best of our knowledge (and surprise), this question is not addressed in the literature, and we believe that our result improves our understanding of the membership parameter for the dominating set problem and adds to the line of results in~\cite{Chapelle10}.
%(number of times any vertex gets dominated).
\begin{table}[]
\label{tab:table1}
\begin{threeparttable}[b]
\caption{Comparison of Parameterized algorithms for problems related to MMDS}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Problem}                                                                                                         & \textbf{Restriction}                                                                                                                                & \textbf{Parameter}             & \textbf{Complexity}                                   \\ \hline
Perfect Code                                                                                                             &                                                                                                                                                    & Solution Size                  & W{[}1{]}-hard ~\cite{DowneyFellows92} \\ \hline
\multirow{2}{*}{\srds}                                                                                    & \begin{tabular}[c]{@{}l@{}}$\sigma$ and $\rho$ \\ are finite sets\end{tabular}                                                               & Treewidth                      & FPT ~\cite{Chapelle10}                \\ \cline{2-4} 
                                                                                                                         & \begin{tabular}[c]{@{}l@{}}$\sigma$ contains  arbitrarily\\  large gaps between two\\  consecutive elements\\  and $\rho$ is cofinite\end{tabular} & Treewidth                      & W{[}1{]}-hard~\cite{Chapelle10}      \\ \hline
\multirow{2}{*}{\rjds}                                                                                    & $d$-degenerate graphs                                                                                                                              & \multirow{3}{*}{Solution Size} & W{[}1{]}-hard  ~\cite{MeybodiFMP20}   \\ \cline{2-2} \cline{4-4} 
                                                                                                                         & nowhere dense graphs                                                                                                                               &                                & FPT~\cite{MeybodiFMP20}               \\ \cline{1-2} \cline{4-4} 
\begin{tabular}[c]{@{}l@{}}\textsc{Restrained Dominating }\\ \textsc{Set}\end{tabular} & 3-degenerate graphs                                                                                                                                &                                & W{[}1{]}-hard ~\cite{MeybodiFMP20}    \\ \hline
MMDS (this paper)                                                                                                            &  Membership bounded by $k$                                                                                                                                                     & Pathwidth                  & W{[}1{]}-hard \\ \hline
\end{tabular}
%\begin{tablenotes}
 %    \item[1] This paper
 %  \end{tablenotes}
\end{threeparttable}
\end{table}
% Due to lack of space, the detailed related work part is presented in the full paper in the Appendix. \\
%\noindent {\bf Variants of dominating sets.} 



==> twincover.tex <==
\section{Twin cover}
\label{sec:twincover}
This section is dedicated to MMDS parameterized by the minimum twin cover of the input graph $G$. 
We show that this problem admits an FPT algorithm. 
%Later, we show the algorithmic lower bound obtained using ETH on the running time of the FPT algorithm mentioned above.
We construct an FPT-time Turing reduction from MMDS to an instance of Integer Linear Programming (ILP)where the number of variables is bounded by some function of the twin cover. 
The reduction target is the following ILP problem:

\begin{tcolorbox}
Integer Linear Programming\\

\begin{tabular}{llp{9cm}}
\textsf{Input}&:& A matrix $A \in \mathbb{Z}^{m \times \ell}$ and a vector $b \in \mathbb{Z}^m$.\\
{\sf Parameter}&:& $\ell$\\
{\sf Question}&:& Is there a vector $x \in \mathbb{Z}^{\ell}$ such that $A \cdot x \leq b$?
\end{tabular}
\end{tcolorbox}

\begin{theorem}[\cite{Lenstra83}]
ILP can be solved in time $O(\ell^{2.5\ell + o(\ell)} L)$ and space polynomial in $L$ where $L$ is the number of bits in the input. 
\end{theorem}

Let $\tc$ be the minimum size of a twin cover of the input graph $G$. 
Our FPT-time Turing reduction constructs at most $2^{O(\tc)}$ instances of ILP in time $2^{O(\tc)}n^{O(1)}$. 
Each instance of the ILP has $\ell = 2^{O(\tc)}$. 
Moreover, at least one fo the constructed instances of ILP is a yes instance if and only if one can show that $\langle G, k\rangle$ is a yes instance of MMDS. 

\begin{theorem}[\cite{Ganian16}]
\label{thm:tcalgo}
If a minimum twin cover in $G$ has size at most $k$, then it is possible to find a twin cover of size $k$ in time $O(|E|+k|V|+ 1.2738^k)$.
\end{theorem}

We start with computing a minimum twin cover $T$ of $G$. 
Using Theorem~\ref{thm:tcalgo}, we can find $T$ (of size $\tc$) in time $O(|E| + \tc|V| + 1.2738^\tc)$. 
We use the following property of $T$ to define a new graph $H$ which is used in our FPT-time Turing reduction. 
$G[V \setminus T]$ is a collection of disjoint cliques. 
Let $D = \{D_1, D_2, \ldots, D_h\}$ be the cliques in $G[V \setminus T]$. 
For each $i \in [h]$, and for each $u,v \in V(D_i)$, $N[u] = n[v]$ since each edge in $E(D_i)$ is a twin edge. 
We construct graph $H$ from $G$ by replacing each clique $D_i$ for $i \in [h]$ by a single vertex $b_i$. 

\subsection{ILP Formulation}
For a subset $C$ of $T$, we ask whether there exists a feasible solution $S$ such that $S \cap T = C$. 
We formulation an ILP instance for the selected subset $C$. 
Let us define the following sets:
\begin{itemize}
\item $X = \{b_i \mid N(b_i) \cap C = \emptyset, \text{ for } i \in [h]\}$
\item 
\end{itemize}
